Hijacking Context in Large Multi-modal Models

Recently, Large Multi-modal Models (LMMs) have demonstrated their ability to understand the visual contents of images given the instructions regarding the images. Built upon the Large Language Models (LLMs), LMMs also inherit their abilities and characteristics such as in-context learning where a coherent sequence of images and texts are given as the input prompt. However, we identify a new limitation of off-the-shelf LMMs where a small fraction of incoherent images or text descriptions mislead LMMs to only generate biased output about the hijacked context, not the originally intended context. To address this, we propose a pre-filtering method that removes irrelevant contexts via GPT-4V, based on its robustness towards distribution shift within the contexts. We further investigate whether replacing the hijacked visual and textual contexts with the correlated ones via GPT-4V and text-to-image models can help yield coherent responses.

==> figures/method_remove.tex <==
\begin{figure*}[t]
    \centering
    % \includegraphics[width=1\linewidth]{figures/overview}
    % \includegraphics[width=1\linewidth]{figures/overview_updated}
    \includegraphics[width=1.05\linewidth]{figures/method_remove.png}

    \vspace{4mm}
    \caption{\textbf{Filtering hijacked contexts via GPT-4(V).} Given multiple image-text pairs of a visual story plot from VIST dataset~\cite{vist}, GPT-4 is instructed to filter any irrelevant images or text descriptions based on the context.
    }
    \vspace{3mm}
    \label{fig:method_remove}
\end{figure*}

==> manuscripts/4_Method.tex <==

\section{Method}
\label{sec:method}

\paragraph{Filtering hijacked contexts.}
To address the context hijacking issue, we first propose a simple yet effective method that can preemptively remove hijacked visual or textual contexts. We observed that GPT-4 and GPT-4V have the capability to filter irrelevant textual or visual contexts via a simple few-shot prompting, based on the powerful zero-shot performance and its robustness towards distribution shift within the contexts. As in Figure \ref{fig:method_remove}, we labeled the sequence number for each image for GPT-4 to understand both the image and text pair correspondingly. Then, we prompted GPT-4 to remove any irrelevant images or textual contexts based on the story plot. GPT-4 appropriately identifies the hijacked contexts (sequence number 5) and hence these filtered outputs will prevent LMMs (such as FROMAGe) from yielding hijacked responses.

\input{figures/method_remove}

\paragraph{Reforming hijacked contexts} We further investigate whether reforming the identified irrelevant visual and textual contexts into coherent ones can help LMMs yield better coherent responses. As in Figure \ref{fig:method_reform}, to reform the hijacked text description, we first instructed GPT-4 to provide appropriate sentences that convey coherency given in the contexts. Subsequently, we instructed DALLE-3 to generate a synthetic image that corresponds to the newly reformed text, with the consideration of underlying visual and textual context information. Consequently, the arranged sequence of visual and textual contexts with the newly reformed one might help to provide a more sufficient and coherent context for LMMs not to be confused.


\input{figures/method_reform}

% GPT-4의 Robustness 얘기 (incoherent context에 대해서 robust하다. w/ & w/o incoherent context 결과 그림). 이는 GPT-4를 써서 filtering 혹은 replacing하는 framework를 구성하겠다는 근거 빌드업을 위함임.

% overall framework에 대한 그림 (filtering, replacing)

% 두가지 측면에서 접근해본다.
% Subsection 1: Filtering에 관해..
    % Solution 1. Can GPT-4 filter out these hijacked-texts?
        % prompt 소개
    % Solution 2. Can GPT-4 filter out these hijacked-images?
        % prompt 소개
% Subsection: Replacing에 관해.
    % Hijacked-text => text with Better Context via GPT-4 prompting?
        % prompt 소개
    % Hijacked-Image => Image with Better Context via text-to-image models? Dall-e?
        % prompt 소개
